Inv-Adapter: ID Customization Generation via Image Inversion and Lightweight Adapter

The remarkable advancement in text-to-image generation models significantly boosts the research in ID customization generation. However, existing personalization methods cannot simultaneously satisfy high fidelity and high-efficiency requirements. Their main bottleneck lies in the prompt image encoder, which produces weak alignment signals with the text-to-image model and significantly increased model size. Towards this end, we propose a lightweight Inv-Adapter, which first extracts diffusion-domain representations of ID images utilizing a pre-trained text-to-image model via DDIM image inversion, without additional image encoder. Benefiting from the high alignment of the extracted ID prompt features and the intermediate features of the text-to-image model, we then embed them efficiently into the base text-to-image model by carefully designing a lightweight attention adapter. We conduct extensive experiments to assess ID fidelity, generation loyalty, speed, and training parameters, all of which show that the proposed Inv-Adapter is highly competitive in ID customization generation and model scale.

==> section/00abs.tex <==
\begin{abstract}
  The remarkable advancement in text-to-image generation models significantly boosts the research in ID customization generation. 
  %
  However, existing personalization methods cannot simultaneously satisfy high fidelity, flexible editing, and high-efficiency requirements. 
  %
  Their main bottleneck lies in the prompt image encoder, which produces weak alignment signals with the text-to-image model, and thus the extracted features cannot be seamlessly embedded into the text-to-image model.
  %
  Towards this end, we propose Inv-Adapter, which first extracts diffusion-domain representations of ID images from a pre-trained text-to-image model via DDIM image inversion. Benefiting from the high alignment of the extracted ID prompt features and the intermediate features of the text-to-image model, we then embed them efficiently into the base text-to-image model by carefully designing a lightweight attention adapter. 
  %
  We conduct extensive experiments to assess ID fidelity, generation loyalty, speed, and training parameters, all of which show that the proposed Inv-Adapter is highly competitive in ID customization generation and model scale.
  \keywords{ID Customization Generation \and Embedded Attention Adapter \and Image Inversion \and Text-to-Image Generation}
\end{abstract}

% The remarkable advancement in text-to-image generation models significantly boosts the research in ID customization generation. However, existing personalization methods cannot simultaneously satisfy high fidelity, flexible editing, and high-efficiency requirements. Their main bottleneck lies in the prompt image encoder, which produces weak alignment signals with the text-to-image model, and thus the extracted features cannot be seamlessly embedded into the text-to-image model. Towards this end, we propose Inv-Adapter, which first extracts diffusion-domain representations of ID images from a pre-trained text-to-image model via DDIM image inversion. Benefiting from the high alignment of the extracted ID prompt features and the intermediate features of the text-to-image model, we then embed them efficiently into the base text-to-image model by carefully designing a lightweight attention adapter. We conduct extensive experiments to assess ID fidelity, generation loyalty, speed, and training parameters, all of which show that the proposed Inv-Adapter is highly competitive in ID customization generation.
